Harmful Speech Detection by Language Models Exhibits Gender-Queer Dialect Bias

Content moderation on social media platforms shapes the dynamics of online discourse, influencing whose voices are amplified and whose are suppressed. Recent studies have raised concerns about the fairness of content moderation practices, particularly for aggressively flagging posts from transgender and non-binary individuals as toxic. In this study, we investigate the presence of bias in harmful speech classification of gender-queer dialect online, focusing specifically on the treatment of reclaimed slurs. We introduce a novel dataset, QueerReclaimLex, based on 109 curated templates exemplifying non-derogatory uses of LGBTQ+ slurs. Dataset instances are scored by gender-queer annotators for potential harm depending on additional context about speaker identity. We systematically evaluate the performance of five off-the-shelf language models in assessing the harm of these texts and explore the effectiveness of chain-of-thought prompting to teach large language models (LLMs) to leverage author identity context. We reveal a tendency for these models to inaccurately flag texts authored by gender-queer individuals as harmful. Strikingly, across all LLMs the performance is poorest for texts that show signs of being written by individuals targeted by the featured slur (F1 <= 0.24). We highlight an urgent need for fairness and inclusivity in content moderation systems. By uncovering these biases, this work aims to inform the development of more equitable content moderation practices and contribute to the creation of inclusive online spaces for all users.

==> intro_old_4.5.24.tex <==
% online communities are HUGE for LGBTQ+ community. Given the legacy of transgender erasure, these systems are crucial for building healthy gender identity.
%Online communities often function as a safe space for LGBTQ+ members. 

% Content moderation determines who is seen and who is allowed to participate in online systems. We have already seen the transphobia continued into tech through weird content moderation practices.
%\textcolor{red}{[For motivation, emphasize the importance of content moderation for safer, more welcoming communities.]}
%A top priority for online creators in content moderation is equality among peers \cite{Ma_Kou_2022}, however s
Social media can be a strong tool to build community and share experiences, though bad actors often infiltrate these spaces with harassment and hate speech.
There is potential for content moderation to play a key role in creating safe and welcoming online environments.
Previously, automated content moderation has been performed by binary classifiers, though computational scientists are now pivoting towards developing content moderation approaches using large language models (LLMs) (e.g. \cite{kumar2023watch, kwon2023efficacy}).

Unfortunately, a growing body of research suggests that social media platforms remove posts and ban users in manners which amplify systemic power %ly unfair power structures %injustices and amplify unfair power structures 
\cite{Shahid_Vashistha_2023, Harris_Johnson_Palmer_Yang_Bruckman_2023}.
In particular, content posted by the transgender community are disproportionately wrongly moderated for portraying `adult' content, criticizing existing power structures, and discussing queer issues  \cite{Haimson_Delmonaco_Nie_Wegner_2021}.
Likewise, when measured by the same toxicity algorithm that moderates the New York Times comments section, tweets from past RuPaul's Drag Race contestants score higher for toxicity than white nationalists \cite{Dias}.
%Online discussions promote the well-being of historically marginalized communities, life satisfaction and even civic engagement \cite{pendry2015individual}. 
These studies suggest that content moderation algorithms broadly contribute to the censorship of trans and non-binary people \cite{namaste2000invisible, scheuerman2021auto}, however the mechanisms for this discrimination are largely unknown. 


Online communities are crucial for %emerging and `elder' members of 
the gender-queer (dnon-socially normative gender identity) community in particular. 
Transgender adolescents use online communities for emotional and information support \cite{selkie2020transgender}, as well as for experimenting with gender identity and navigating the challenges of coming out \cite{herrmann2023social}.
In fact, LGTBQ+ youth have been found to be more likely to participate in online communities over those in real life~\cite{mcinroy2019lgbtq}.
We know that gender-queer populations are at a higher risk of discrimination, mortality, social isolation, and homelessness ~\cite{tabaac2018discrimination, mccann2021homeless}. %, and are at higher risk for experiencing homelessness \cite{mccann2021homeless}.
Particularly in areas where support for LGBTQ+ individuals is limited, queer online spaces are crucial for healthy and happy lives.


%Online communities are crucial for emerging and `elder' members of the gender-queer (LGBTQ+) community. Transgender adolescents use online communities for emotional and information support \cite{selkie2020transgender}, as well as for experimenting with gender identity and navigating the challenges of coming out \cite{herrmann2023social}. In fact, LGTBQ+ youths have been found to be more likely to participate in online LGBTQ+ communities than those in real life\cite{mcinroy2019lgbtq}. At the same time, gender-queer populations are at a higher risk of discrimination, mortality, and social isolation~\cite{tabaac2018discrimination}, and are at higher risk for experiencing homelessness \cite{mccann2021homeless}. Particularly in areas where support for LGBTQ+ individuals is limited, queer online spaces are crucial for healthy and happy lives.

%There is a growing body of research suggesting that social media platforms remove posts and ban users in manners which amplify historical inequity %ly unfair power structures %injustices and amplify unfair power structures \cite{Shahid_Vashistha_2023, Harris_Johnson_Palmer_Yang_Bruckman_2023}.In particular,  content posted by transgender community is disproportionately removed for portraying `adult' content, criticizing existing power structures, and discussing queer issues  \cite{Haimson_Delmonaco_Nie_Wegner_2021}. Meanwhile, Twitter users with non-binary pronouns in their biography are flagged for toxicity at higher rates than users with binary pronouns and also receive less engagement with their posts in the form of  retweets and likes \cite{dorn2023non}. Likewise, when measured by the same toxicity algorithm that moderates the New York Times comments section, tweets from past RuPaul's Drag Race contestants score higher for toxicity than white nationalists \cite{Dias}.
%These studies suggest that content moderation algorithms broadly contribute to the censorship of trans and non-binary people \cite{namaste2000invisible, scheuerman2021auto}, however the mechanisms for this discrimination are largely unknown. 

%Previous work found that Twitter users with non-binary pronouns in their biography are flagged for toxicity at higher rates than users with binary pronouns, also receive less engagement with their posts in the form of  retweets and likes \cite{dorn2023non}.
A prominent practice of gender-queer group dialect is \textbf{linguistic reclamation} \cite{Edmondson_2021, worthen2020queers} which refers to
``non-derogatory uses, by members of marginalised groups, of the slurs used by members of hegemonically powerful groups to derogate them" \cite{Edmondson_2021}. 
The gender-queer community has a strong history with linguistic reclamation.
Despite its pejorative past, the term `queer' is more frequently used as an LGBTQ+ descriptor than `gay' in in academic spaces \cite{baker2013gay} and is now commonly included within the `LGBTQ+' acronym. 
The term `femboy' has transformed from being widely understood as a typically pornographic term to a word referencing masculine or assigned male at birth persons presenting themselves with aspects of historically feminine presentation \cite{vytniorgu2023effeminate, anzani2021being, gilbert2020sissy}. In fact, `femboy' now describes a pocket of femme-presenting men on TikTok that is often celebrated for its normalization of gender-variance \cite{foster2022muscles}.

%The gender-queer community has unique linguistic styles like any other social group: Non-binary individuals adopt similar language to nearby gender non-conforming folks \cite{steele2019non} and \becca{source for binary trans people?}. 


%In a survey of Bangladeshi Facebook users who had content removed, majority of respondents agreed that Facebook's content moderation system continues historical injustices and amplifies power structures \cite{Shahid_Vashistha_2023}.
%Transgender people are among the most popular to have their content removed, particularly for 'adult' content, critiques of historically oppressive groups and conversations of queer issues \cite{Haimson_Delmonaco_Nie_Wegner_2021}.
%On Reddit's r/FTM, there is no streamlined process to inform users why their content was taken down though page moderators may communicate with users if they choose to \cite{Thach_Mayworm_Delmonaco_Haimson_2022}.
%In addition to outright user or post removal, demoting a user in algorithm rankings is also a harmful form of content moderation \cite{Gillespie_2022}.
%When Black creators in TikTok are treated unfairly by the algorithms, it continues a legacy of unequal opportunity for Black people \cite{Harris_Johnson_Palmer_Yang_Bruckman_2023}.


% We seek to understand the extend of anti genderqueer dialect bias in large language models. We look at how large language models interact with reclaimed slurs, and whether the bias can be lightened with chain of thought prompting. Research questions go here.
Previous work found that Twitter users with non-binary pronouns in their biography received low amounts of attention on Twitter through retweets and likes, and are flagged for toxicity at alarmingly high rates \cite{dorn2023non}. 
Our goal in this paper is to understand to what extent this disparate treatment is due to a \textit{dialect bias} against gender-queer social media users.
%We measure gender-queer dialect through \textbf{linguistic reclamation} which refers to ``non-derogatory uses, by members of marginalised groups, of the slurs used by members of hegemonically powerful groups to derogate them" \cite{Edmondson_2021}. 

We hypothesize that the language modeling component of content moderation algorithms will have a severely limited capacity for understanding slurs, which appear in both gender-queer dialects \textit{and} hate speech, resulting in higher false-positive rates for toxicity.
Our research questions are as follows:
\begin{itemize}
    \item How do large language models perceive harm of %single
    social media posts featuring reclaimed slurs?
    \item %Do large language models change their understanding of harm depending on author identity context?
    How does additional context about author identity alter how large language models score harm?
    \item% Can large language models learn to respect uses of reclaimed LGBTQ+ slurs through chain-of-thought prompting?
    Can chain-of-thought explanations be leveraged towards improving large language models understanding of LGBTQ+ reclaimed slurs?
\end{itemize}

%\textcolor{red}{[Why LLMs? You had not mentioned them up til now, how do you motivate them now? LLMs should be easy to justify - they are roaring into every aspect of life. But you need to make the link to content moderation directly - or maybe reframe the motivation.]}

In this study, we introduce \dataset$:$ a dataset of naturalistic uses of reclaimed slurs based on real text written by gender-queer authors. Six gender-queer annotators label the dataset for harm two times reflecting different context on author identity.
We test five off-the-shelf language model's abilities to calculate harm and how this ability changes with author identity context and chain-of-thought prompting.
We find that the models frequently falsely flag texts written by gender-queer authors as harmful, and that this performance improves but remains poor when chain-of-thought is used in prompting. 
Further, we observe significantly worse performance on instances with clear markers of gender-queer authorship.
This work identifies a need for models to use in-text context rather than be reliant on slurs as keywords. Further, by finding evidence of high false positive rates towards reclaimed slurs, we highlight a potential risk of large language models posing bias to gender-queer populations.
We hope this work will help inform developers and policy makers in shaping future content moderation systems.

==> tables/change.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{lllll}
                        &                                                               &                                                    & \multicolumn{2}{c}{\contextcot}                                                       \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{}                                         & \multicolumn{1}{l|}{}                              & \multicolumn{1}{l|}{True}                        & \multicolumn{1}{l|}{False}                        \\ \cline{3-5} 
\multicolumn{1}{c}{}    & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{GPT 3.5}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}True}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}346} & \multicolumn{1}{l|}{157}                          \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}False} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}38}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}901}  \\ \cline{3-5} 
\context & \multicolumn{1}{l|}{\textbf{Llama 2}}                         & \multicolumn{1}{l|}{True}                          & \multicolumn{1}{l|}{270}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{9AFF99}396}  \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{}                                         & \multicolumn{1}{l|}{False}                         & \multicolumn{1}{l|}{6}                           & \multicolumn{1}{l|}{770}                          \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Mistral}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}True}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}89}  & \multicolumn{1}{l|}{86}                           \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}False} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}49}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}1218} \\ \cline{3-5} 
\end{tabular}
\caption{Change between \context harm scores and \contextcot harm scores for each model.}
\end{table}

==> tables/change2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{lllll}
                        &                                                               &                                                    & \multicolumn{2}{c}{\contextcot}                                                       \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{}                                         & \multicolumn{1}{l|}{}                              & \multicolumn{1}{l|}{True}                        & \multicolumn{1}{l|}{False}                        \\ \cline{3-5} 
\multicolumn{1}{c}{}    & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{GPT 3.5}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}True}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.24} & \multicolumn{1}{l|}{.11}                          \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}False} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.03}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.62}  \\ \cline{3-5} 
\context & \multicolumn{1}{l|}{\textbf{Llama 2}}                         & \multicolumn{1}{l|}{True}                          & \multicolumn{1}{l|}{.19}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{9AFF99}.27}  \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{}                                         & \multicolumn{1}{l|}{False}                         & \multicolumn{1}{l|}{.01}                           & \multicolumn{1}{l|}{.53}                          \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Mistral}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}True}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.06}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}.06}                           \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}False} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}.03}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.84} \\ \cline{3-5} 
\end{tabular}
\caption{Change between \harmfulifin$\ $scores between \context$\ $ and \contextcot$\ $ prompting schemas.}
\end{table}

==> tables/change_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

\begin{table*}[ht!]
\begin{tabular}{lllllll}
                           & \multicolumn{6}{c}{\contextcot}                                                                                                                                            \\
\multicolumn{1}{c}{}       &                           &    & \multicolumn{2}{l|}{\harmfulifin}                                               & \multicolumn{2}{l}{\harmfulifout}                          \\
                           &                           &    & Harmful                          & \multicolumn{1}{l|}{$\neg$Harmful}                          & Harmful                          & $\neg$Harmful                         \\ \cline{2-7} 
                           &                           & Harmful & \cellcolor[HTML]{EFEFEF}.24 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.11} & \cellcolor[HTML]{C0C0C0}.35 & \cellcolor[HTML]{C0C0C0}.28 \\
                           & \multirow{-2}{*}{GPT 3.5} & $\neg$Harmful& \cellcolor[HTML]{EFEFEF}.03 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.62} & \cellcolor[HTML]{C0C0C0}.01 & \cellcolor[HTML]{C0C0C0}.36 \\ \cline{2-7} 
                           &                           & Harmful & \cellcolor[HTML]{C0C0C0}.19 & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}.27} & \cellcolor[HTML]{EFEFEF}.61 & \cellcolor[HTML]{EFEFEF}.11 \\
                           & \multirow{-2}{*}{Llama 2} & $\neg$Harmful& \cellcolor[HTML]{C0C0C0}.01 & \multicolumn{1}{l|}{\cellcolor[HTML]{C0C0C0}.53} & \cellcolor[HTML]{EFEFEF}.07 & \cellcolor[HTML]{EFEFEF}.21 \\ \cline{2-7} 
                           &                           & Harmful & \cellcolor[HTML]{EFEFEF}.06 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.06} & \cellcolor[HTML]{C0C0C0}.15 & \cellcolor[HTML]{C0C0C0}0   \\
\multirow{-6}{*}{\context} & \multirow{-2}{*}{Mistral} & $\neg$Harmful& \cellcolor[HTML]{EFEFEF}.03 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.84} & \cellcolor[HTML]{C0C0C0}.25 & \cellcolor[HTML]{C0C0C0}.59
\end{tabular}
\caption{A confusion matrix of how Harmful and Not Harmful ($\neg$Harmful) predictions change between \context and \contextcot prompting schemas. 
The diagonal cells in each group of 4 (shown with shades of grey) show the percent of instances for which prediction remains the same. Non-diagonal cells shows shifted predictions.}
\label{tab:changeall2}
\end{table*}

==> tables/change_all2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{cllllll}
\multicolumn{1}{l}{}                                                    &                                       &                            & \multicolumn{4}{l}{\contextcot}                                                                                                                                                            \\ \cline{2-7} 
\multicolumn{1}{l|}{}                                                   & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}      & \multicolumn{2}{l|}{\harmfulifin}                                                    & \multicolumn{2}{l|}{\harmfulifout}                                                   \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                   & \multicolumn{1}{c|}{\textbf{}}        & \multicolumn{1}{l|}{}      & \multicolumn{1}{l|}{True}                        & \multicolumn{1}{l|}{False}                       & \multicolumn{1}{l|}{True}                        & \multicolumn{1}{l|}{False}                       \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                   & \multicolumn{1}{l|}{\textbf{GPT 3.5}} & \multicolumn{1}{l|}{True}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.24} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.11} & \multicolumn{1}{l|}{.35}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFC9E}.28} \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                   & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{False} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.03} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.62} & \multicolumn{1}{l|}{.01}                         & \multicolumn{1}{l|}{.36}                         \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                   & \multicolumn{1}{l|}{\textbf{Llama 2}} & \multicolumn{1}{l|}{True}  & \multicolumn{1}{l|}{.19}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}.27} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.61} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.11} \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                   & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{False} & \multicolumn{1}{l|}{.01}                         & \multicolumn{1}{l|}{.53}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.07} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.21} \\ \cline{2-7} 
\multicolumn{1}{c|}{}                                                   & \multicolumn{1}{l|}{\textbf{Mistral}} & \multicolumn{1}{l|}{True}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.06} & \multicolumn{1}{l|}{\cellcolor[HTML]{96FFFB}.06} & \multicolumn{1}{l|}{.15}                         & \multicolumn{1}{l|}{0}                           \\ \cline{2-7} 
\multicolumn{1}{c|}{\multirow{-7}{*}{\textbf{\context}}
\end{picture}}} & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{False} & \multicolumn{1}{l|}{\cellcolor[HTML]{96FFFB}.03} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.84} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCE93}.25} & \multicolumn{1}{l|}{.59}                         \\ \cline{2-7} 
\multicolumn{1}{l}{}                                                    &                                       &                            &                                                  &                                                  &                                                  &                                                 
\end{tabular}
\caption{How harm predictions change between \context\ and \contextcot\ prompting schemas. Percent of instances}
\label{tab:changeall}
\end{table}

==> tables/change_all_OLD.tex <==
\begin{table}[]
\setlength{\belowcaptionskip}{-10pt}
%\footnotesize
\begin{tabular}{lllllll}
                                             &                                       &                            & \multicolumn{4}{l}{\contextcot}                                                                                                                                                            \\ \cline{2-7} 
\multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}      & \multicolumn{2}{l|}{\harmfulifin}                                                    & \multicolumn{2}{l|}{\harmfulifout}                                                   \\ \cline{2-7} 
\multicolumn{1}{c|}{\textbf{}}               & \multicolumn{1}{c|}{\textbf{}}        & \multicolumn{1}{l|}{}      & \multicolumn{1}{l|}{True}                        & \multicolumn{1}{l|}{False}                       & \multicolumn{1}{l|}{True}                        & \multicolumn{1}{l|}{False}                       \\ \cline{2-7} 
\multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{\textbf{GPT 3.5}} & \multicolumn{1}{l|}{True}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.24} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.11} & \multicolumn{1}{l|}{.35}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.28} \\ \cline{2-7} 
\multicolumn{1}{l|}{\context} & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{False} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.03} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.62} & \multicolumn{1}{l|}{.01}                         & \multicolumn{1}{l|}{.36}                         \\ \cline{2-7} 
\multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{\textbf{Llama 2}} & \multicolumn{1}{l|}{True}  & \multicolumn{1}{l|}{.19}                         & \multicolumn{1}{l|}{.27} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.61} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.11} \\ \cline{2-7} 
\multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{False} & \multicolumn{1}{l|}{.01}                         & \multicolumn{1}{l|}{.53}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.07} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.21} \\ \cline{2-7} 
\multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{\textbf{Mistral}} & \multicolumn{1}{l|}{True}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.06} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.06} & \multicolumn{1}{l|}{.15}                         & \multicolumn{1}{l|}{0}                           \\ \cline{2-7} 
\multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{False} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.03} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.84} & \multicolumn{1}{l|}{.25} & \multicolumn{1}{l|}{.59}                         \\ \cline{2-7} 
                                             &                                       &                            &                                                  &                                                  &                                                  &                                                 
\end{tabular}
\caption{Percent of instances that change between \context\ and \contextcot\ prompting schemas. Percent of instances}
\label{tab:changeall}
\end{table}


==> tables/change_out.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{lllll}
                        &                                                               &                                                    & \multicolumn{2}{c}{\contextcot}                                                      \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{}                                         & \multicolumn{1}{l|}{}                              & \multicolumn{1}{l|}{True}                        & \multicolumn{1}{l|}{False}                       \\ \cline{3-5} 
\multicolumn{1}{c}{}    & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{GPT 3.5}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}True}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.35} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AFF99}.28} \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}False} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.01} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.36} \\ \cline{3-5} 
\context & \multicolumn{1}{l|}{\textbf{Llama 2}}                         & \multicolumn{1}{l|}{True}                          & \multicolumn{1}{l|}{.61}                         & \multicolumn{1}{l|}{.11}                         \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{}                                         & \multicolumn{1}{l|}{False}                         & \multicolumn{1}{l|}{.07}                         & \multicolumn{1}{l|}{.21}                         \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Mistral}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}True}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.15} & \multicolumn{1}{l|}{0}                           \\ \cline{3-5} 
                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}False} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}.25} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}.59} \\ \cline{3-5} 
\end{tabular}
\caption{How \harmfulifout predictions change between \context\ and \contextcot prompting schemas.}
\end{table}

==> tables/linreg_slur.tex <==
\begin{table}[]
\small
\begin{tabular}{l|l|l|l|l|}
\cline{2-5}
                                                                   & \textbf{Human} & \textbf{GPT} & \textbf{Llama} & \textbf{Mistral} \\ \hline
\multicolumn{1}{|l|}{Zeroshot}                            & -              & .220         & .190           & .252             \\ \hline
\multicolumn{1}{|l|}{Ingroup \context}     & .005           & .171         & .154           & .093             \\ \hline
\multicolumn{1}{|l|}{Ingroup \contextcot}  & -              & .080         & .050           & .032             \\ \hline
\multicolumn{1}{|l|}{Outgroup \context}    & .035           & .223         & .107           & .130             \\ \hline
\multicolumn{1}{|l|}{Outgroup \contextcot} & -              & .138         & .106           & .072             \\ \hline
\end{tabular}
\caption{Linear Regression R-Squared statistics measuring correlation between model harm scores and slur featured in template. For all regressions, p $<$ .01. \becca{Change heirarchy of terms (harmful if in -> identity} \textcolor{red}{sorry to be annoying but should this be the only table where the models are columns?}}
\label{tab:linreg_slur}
\end{table}

==> tables/linreg_slur_2.tex <==
\begin{table*}[]
\begin{tabular}{ll|ll|ll|}
\cline{3-6}
                                       &                           & \multicolumn{2}{l|}{\harmfulifin}                          & \multicolumn{2}{l|}{\harmfulifout}                         \\ \cline{2-6} 
\multicolumn{1}{l|}{}                  & \nocontext & \multicolumn{1}{l|}{\context} & \contextcot & \multicolumn{1}{l|}{\context} & \contextcot \\ \hline
\multicolumn{1}{|l|}{\textbf{Human}}   & -                         & \multicolumn{1}{l|}{.005}                    & -                          & \multicolumn{1}{l|}{.035}                    & -                          \\ \hline
\multicolumn{1}{|l|}{\textbf{GPT 3.5}} & .220                      & \multicolumn{1}{l|}{.171}                    & .080                       & \multicolumn{1}{l|}{.223}                    & .138                       \\ \hline
\multicolumn{1}{|l|}{\textbf{Llama 2}} & .190                      & \multicolumn{1}{l|}{.154}                    & .050                       & \multicolumn{1}{l|}{.107}                    & .106                       \\ \hline
\multicolumn{1}{|l|}{\textbf{Mistral}} & .252                      & \multicolumn{1}{l|}{.093}                    & .032                       & \multicolumn{1}{l|}{.130}                    & .072                       \\ \hline
\end{tabular}
\caption{Linear Regression R-Squared statistics measuring correlation between model harm scores and slur featured in template. For all regressions, p $<$ .01.}
\label{tab:linreg_slur}
\end{table*}

==> tables/linreg_slurusage.tex <==
\begin{table}[]
\small
\begin{tabular}{l|l|l|l|l|}
\cline{2-5}
                                                                   & \textbf{Human} & \textbf{GPT} & \textbf{Llama} & \textbf{Mistral} \\ \hline
\multicolumn{1}{|l|}{Zeroshot}                            & -              & .660        & .740           & .593             \\ \hline
\multicolumn{1}{|l|}{Ingroup \context}     & .238           & .495         & .767           & .440             \\ \hline
\multicolumn{1}{|l|}{Ingroup \contextcot}  & -              & .468         & .778           & .207             \\ \hline
\multicolumn{1}{|l|}{Outgroup \context}    & .779           & .750         & .847           & .638            \\ \hline
\multicolumn{1}{|l|}{Outgroup \contextcot} & -              & .515         & .873           & .515             \\ \hline
\end{tabular}
\caption{Linear Regression R-Squared statistics measuring correlation between model harm scores and \slurtype. For all regressions, p $<$ .01.}
\end{table}

==> tables/model_table4.tex <==
\begin{table*}[]
\small
\begin{tabular}{l|lllllllll|lllllllll|}
\cline{2-19}
                                           & \multicolumn{9}{c|}{\textbf{INGROUP (n=752)}}                                                                                                                                                                                                         & \multicolumn{9}{c|}{\textbf{OUTGROUP (n=641)}}                                                                                                                                                                                                        \\ \cline{2-19} 
                                           & \multicolumn{3}{l|}{\nocontext}                                                & \multicolumn{3}{l|}{\context}                                                            & \multicolumn{3}{l|}{\contextcot}                                   & \multicolumn{3}{l|}{\nocontext}                                                & \multicolumn{3}{l|}{\context}                                                            & \multicolumn{3}{l|}{\contextcot}                                   \\ \cline{2-19} 
                                           & \multicolumn{1}{l|}{P}   & \multicolumn{1}{l|}{R}   & \multicolumn{1}{l|}{F1}  & \multicolumn{1}{l|}{P}   & \multicolumn{1}{l|}{R}   & \multicolumn{1}{l|}{F1}           & \multicolumn{1}{l|}{P}   & \multicolumn{1}{l|}{R}   & F1           & \multicolumn{1}{l|}{P}   & \multicolumn{1}{l|}{R}   & \multicolumn{1}{l|}{F1}  & \multicolumn{1}{l|}{P}   & \multicolumn{1}{l|}{R}   & \multicolumn{1}{l|}{F1}           & \multicolumn{1}{l|}{P}   & \multicolumn{1}{l|}{R}   & F1           \\ \hline
\multicolumn{1}{|l|}{\textbf{Detoxify}}    & \multicolumn{1}{l|}{.13} & \multicolumn{1}{l|}{.62} & \multicolumn{1}{l|}{.23} & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}            & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}   & -            & \multicolumn{1}{l|}{.80} & \multicolumn{1}{l|}{.49} & \multicolumn{1}{l|}{.60} & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}            & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}   & -            \\ \hline
\multicolumn{1}{|l|}{\textbf{Perspective}} & \multicolumn{1}{l|}{.19} & \multicolumn{1}{l|}{.47} & \multicolumn{1}{l|}{.26} & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}            & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}   & -            & \multicolumn{1}{l|}{.82} & \multicolumn{1}{l|}{.27} & \multicolumn{1}{l|}{.41} & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}            & \multicolumn{1}{l|}{-}   & \multicolumn{1}{l|}{-}   & -            \\ \hline
\multicolumn{1}{|l|}{\textbf{GPT-3.5}}     & \multicolumn{1}{l|}{.16} & \multicolumn{1}{l|}{.96} & \multicolumn{1}{l|}{.27} & \multicolumn{1}{l|}{.21} & \multicolumn{1}{l|}{.91} & \multicolumn{1}{l|}{.34}          & \multicolumn{1}{l|}{.28} & \multicolumn{1}{l|}{.89} & \textbf{.43} & \multicolumn{1}{l|}{.84} & \multicolumn{1}{l|}{.68} & \multicolumn{1}{l|}{.75} & \multicolumn{1}{l|}{.85} & \multicolumn{1}{l|}{.85} & \multicolumn{1}{l|}{\textbf{.85}} & \multicolumn{1}{l|}{.88} & \multicolumn{1}{l|}{.55} & .67          \\ \hline
\multicolumn{1}{|l|}{\textbf{Llama2}}      & \multicolumn{1}{l|}{.17} & \multicolumn{1}{l|}{.88} & \multicolumn{1}{l|}{.29} & \multicolumn{1}{l|}{.17} & \multicolumn{1}{l|}{.91} & \multicolumn{1}{l|}{.29}          & \multicolumn{1}{l|}{.36} & \multicolumn{1}{l|}{.76} & \textbf{.49} & \multicolumn{1}{l|}{.83} & \multicolumn{1}{l|}{.55} & \multicolumn{1}{l|}{.66} & \multicolumn{1}{l|}{.83} & \multicolumn{1}{l|}{.82} & \multicolumn{1}{l|}{\textbf{.83}} & \multicolumn{1}{l|}{.85} & \multicolumn{1}{l|}{.82} & \textbf{.83} \\ \hline
\multicolumn{1}{|l|}{\textbf{Mistral}}     & \multicolumn{1}{l|}{.21} & \multicolumn{1}{l|}{.66} & \multicolumn{1}{l|}{.32} & \multicolumn{1}{l|}{.28} & \multicolumn{1}{l|}{.43} & \multicolumn{1}{l|}{\textbf{.34}} & \multicolumn{1}{l|}{.31} & \multicolumn{1}{l|}{.30} & .30          & \multicolumn{1}{l|}{.81} & \multicolumn{1}{l|}{.34} & \multicolumn{1}{l|}{.48} & \multicolumn{1}{l|}{.77} & \multicolumn{1}{l|}{.20} & \multicolumn{1}{l|}{.32}          & \multicolumn{1}{l|}{.81} & \multicolumn{1}{l|}{.51} & \textbf{.63} \\ \hline
\end{tabular}
\label{tab:PRF1}
\caption{Precision, Recall and F1 scores for each model with differing prompting context. Column \nocontext refers to zero shot classification scores, \context references ingroup/outgroup classification scores, and \contextcot references chain-of-thought prompting classification scores. Across all models, instances featuring linguistic reclamation are overwhelmingly falsely flagged as harmful.}
\end{table*}

==> tables/mutualinfo_slur.tex <==
\begin{table}[]
\footnotesize
\begin{tabular}{l|l|l|l|l|}
\cline{2-5}
                                                          & \textbf{Human} & \textbf{GPT 3.5} & \textbf{Llama 2} & \textbf{Mistral} \\ \hline
\multicolumn{1}{|l|}{Zeroshot}                            & -              & .149         & .134           & .206             \\ \hline
\multicolumn{1}{|l|}{Ingroup \context}     & .007           & .116         & .118           & .060             \\ \hline
\multicolumn{1}{|l|}{Ingroup \contextcot}  & -              & .063         & .040           & .024             \\ \hline
\multicolumn{1}{|l|}{Outgroup \context}    & .013           & .126         & .088           & .119             \\ \hline
\multicolumn{1}{|l|}{Outgroup \contextcot} & -              & .038         & .058           & .003             \\ \hline
\end{tabular}
\caption{Mutual Information between harm score and slur featured in a template.}
\label{tab:mutinfo_slur}
\end{table}

==> tables/mutualinfo_slurtype.tex <==
\begin{table}[]
\footnotesize
\begin{tabular}{l|l|l|l|l|}
\cline{2-5}
                                                          & \textbf{Human} & \textbf{GPT 3.5} & \textbf{Llama 2} & \textbf{Mistral} \\ \hline
\multicolumn{1}{|l|}{Zeroshot}                            & -              & .079         & .076           & .078             \\ \hline
\multicolumn{1}{|l|}{Ingroup \context}     & .067           & .053         & .059           & .095             \\ \hline
\multicolumn{1}{|l|}{Ingroup \contextcot}  & -              & .088         & .077           & .031             \\ \hline
\multicolumn{1}{|l|}{Outgroup \context}    & .056           & .059         & .047           & .113             \\ \hline
\multicolumn{1}{|l|}{Outgroup \contextcot} & -              & .085         & .027           & .060             \\ \hline
\end{tabular}
\caption{Mutual Information between harm score and \slurtype\ featured in a template.}
\label{tab:mutinfo_slurusage}
\end{table}

==> tables/slurtype_def_table.tex <==
\begin{table*}[h!]
\begin{tabular}{|l|l|l|}
\hline
\textbf{Slur Type}                                               & \textbf{Definition}                                                                                                                                                     & \textbf{Example}                                                                                                                                                   \\ \hline
Neologism                                                         & \begin{tabular}[c]{@{}l@{}}Slur contorted to a new linguistic format, such as \\ using a noun as a verb or creating a new word\\ entirely.\end{tabular}                 & \textit{\begin{tabular}[c]{@{}l@{}}It’s always a good day for \\ dyke frogs.\end{tabular}}                                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}Community\\ Focus\end{tabular}         & A slur which describes a group of people.                                                                                                                               & \textit{\begin{tabular}[c]{@{}l@{}}rainbow flag perfect for \\ some of the queers bc they\\  always acting like clowns\end{tabular}}                               \\ \hline
Stand Alone                                                       & \begin{tabular}[c]{@{}l@{}}Slur is the the only, single or repeated, word in a\\ phrase.*\end{tabular}                                                                  & \textit{tranny!!!!!}                                                                                                                                               \\ \hline
Sexualization                                                     & \begin{tabular}[c]{@{}l@{}}A slur used to focus heavily on sexual appearance, \\ physical beauty, and sexual appeal to others.\end{tabular}                             & \textit{\begin{tabular}[c]{@{}l@{}}I missed watching fags \\ make out in the club\end{tabular}}                                                                    \\ \hline
Self Label                                                        & \begin{tabular}[c]{@{}l@{}}A slur is a self label when the speaker references\\ themselves as a member of the in-group.\end{tabular}                                    & \textit{\begin{tabular}[c]{@{}l@{}}I am the biggest dyke you\\  will ever meet\end{tabular}}                                                                       \\ \hline
Other Label                                                       & A slur ascribed to someone who is not the speaker.                                                                                                                      & \textit{\begin{tabular}[c]{@{}l@{}}He's a fucking shemale is\\ what he is.\end{tabular}}                                                                           \\ \hline
Reclamation                                                       & \begin{tabular}[c]{@{}l@{}}A slur use that places power with in-group \\ members.\end{tabular}                                                                          & \textit{\begin{tabular}[c]{@{}l@{}}Everything can suck, but \\ being a faggot (right) is \\ so fucking cool\end{tabular}}                                          \\ \hline
\begin{tabular}[c]{@{}l@{}}Counter\\ Speech\end{tabular}          & \begin{tabular}[c]{@{}l@{}}A slur responding directly to an instance of \\ derogation, in defense against a comment made \\ by a single speaker or group.*\end{tabular} & \textit{\begin{tabular}[c]{@{}l@{}}@user don't call her a \\ dyke.\end{tabular}}                                                                                   \\ \hline
Quote                                                             & \begin{tabular}[c]{@{}l@{}}Reference to a slur embedded in a quote or \\ paraphrase.\end{tabular}                                                                       & \textit{\begin{tabular}[c]{@{}l@{}}lexi said “stop being\\ a dyke \textless{}3"\end{tabular}}                                                                      \\ \hline
\begin{tabular}[c]{@{}l@{}}Discussion of\\ Slur\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Discussion of a slur, its origin, or acceptable use\\ cases.*\end{tabular}                                                                   & \textit{\begin{tabular}[c]{@{}l@{}}who do they think they \\ are to determine if \\ someone's a tranny or \\ not??\end{tabular}}                                   \\ \hline
\begin{tabular}[c]{@{}l@{}}Discussion of \\ Identity\end{tabular} & \begin{tabular}[c]{@{}l@{}}Discussion of in-group identity dynamics and \\ related concepts.\end{tabular}                                                               & \textit{\begin{tabular}[c]{@{}l@{}}@user gonna be super\\ frank- fags die because \\ we are left out of the \\ healthcare discussion.\end{tabular}}                \\ \hline
Recollection                                                      & Recollection of a time that a slur was used.*                                                                                                                           & \textit{\begin{tabular}[c]{@{}l@{}}Happy pride month to \\ everyone except that one\\ kid who asked if he \\ could call me his dyke at\\ senior prom\end{tabular}} \\ \hline
Sarcasm                                                           & \begin{tabular}[c]{@{}l@{}}A slur used ironically, contrary to its original\\ meaning.*\end{tabular}                                                                    & \textit{\begin{tabular}[c]{@{}l@{}}If yr such an ally why dont\\  u go ahead and say \\ transvestite huh. no really\\  go ahead.\end{tabular}}                     \\ \hline
Homonym                                                           & A slur with one or more non-derogatory meaning.*                                                                                                                        & N/A                                                                                                                                                                \\ \hline
\end{tabular}
\caption{Definitions of each category within the \texttt{SLUR\_TYPE} variable. Asterisk means that the definition is directly taken from \cite{Kurrek_Saleem_Ruths_2020}. Examples are templates from our dataset.}
\label{fig:slur_typedef}
\end{table*}

==> tables/slurtype_examples.tex <==
\begin{table}[]
\footnotesize
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Instance}}                                                                                                                    & \multicolumn{1}{c|}{\textbf{Slur Usage}}                                     \\ \hline
\begin{tabular}[c]{@{}l@{}}Happy pride month, bitches and bros and $[SLUR]$ \\ hoes\end{tabular}                                                            & Group Label                                                             \\ \hline
Dear GOD I wish I had another $[SLUR]$ coworker                                                                                                             & \begin{tabular}[c]{@{}l@{}}Discussion of Identity,\\ Self Label\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Go ahead and cancel your appointment because\\ you "Don't want a $[SLUR]$ " tattooing you, I'm \\ keeping your deposit.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Counter Speech,\\ Recollection\end{tabular}       \\ \hline
\begin{tabular}[c]{@{}l@{}}straight creators stop putting the word $[SLUR]$ in\\ your edgy show/movie challenge 2020\end{tabular}                            & \begin{tabular}[c]{@{}l@{}}Counter Speech,\\ Discussion of Slur\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Not all $[SLUR]$s do coding and stuff, some of us\\ are actually really dumb\end{tabular}                                        & \begin{tabular}[c]{@{}l@{}}Group Label,\\ Sarcasm\end{tabular}           \\ \hline
\end{tabular}
\caption{Examples of templates with corresponding \slurtype framework classifications.}
\label{tab:examples}
\end{table}
